Predicting the Temporal Dynamics of Information Diffusion in Social Networks

Online social networks play a major role in the spread of information at very large scale and it becomes essential to provide means to analyse this phenomenon. In this paper we address the issue of predicting the temporal dynamics of the information diffusion process. We develop a graph-based approach built on the assumption that the macroscopic dynamics of the spreading process are explained by the topology of the network and the interactions that occur through it, between pairs of users, on the basis of properties at the microscopic level. We introduce a generic model, called T-BaSIC, and describe how to estimate its parameters from users behaviours using machine learning techniques. Contrary to classical approaches where the parameters are fixed in advance, T-BaSIC's parameters are functions depending of time, which permit to better approximate and adapt to the diffusion phenomenon observed in online social networks. Our proposal has been validated on real Twitter datasets. Experiments show that our approach is able to capture the particular patterns of diffusion depending of the studied sub-networks of users and topics. The results corroborate the "two-step" theory (1955) that states that information flows from media to a few "opinion leaders" who then transfer it to the mass population via social networks and show that it applies in the online context. This work also highlights interesting recommendations for future investigations.

==> contributions.tex <==
The contributions of this paper are the following:
\begin{enumerate}
\item An analytical discussion about how to detect spreading topics and the features that may explain the diffusion process. This step has been performed using a dataset based on Twitter. It enabled us to understand the overall process of information diffusion in a real social network.
\item A new model for information diffusion modeling in online social networks and a set of features used to estimate its parameters. This new model, \textit{T-BAsIC}, permits a deeper integration of time in the prediction process. The features are based on users behaviour and belong to three dimensions (social, topic, and time).
\item An experimental study that aims to assess the efficiency of our approach and the validity of the underlying assumption (i.e. the macroscopic diffusion process is explained by the sum of microscopic interactions that occur because of local properties).
\end{enumerate}

==> information_diffusion.tex <==
\textbf{Problem definition.} ``Information diffusion'' is a generic concept that refers to all processes of propagation in a system, regardless of the nature of the object in motion. The diffusion of innovation over a network is one of the original reasons for studying networks and the spread of disease among a population has been studied for centuries. The models developed in the context of social networks assume that people are influenced by actions taken by their surrounding, in other words, they are developed under the assumption of ``information cascade''. That is why the path followed by an information in the network is often referred to as the ``spreading cascade''. In the case of Twitter, one can be interested by the spread of particular objects like hashtags or URLs or even broader concepts like topics for instance. Modeling information diffusion first requires to define the set of actors that can potentially be involved. In the context of online social networks, an actor is referred to as a node. The simplest way to describe the spreading process is to consider that a node can be whether active or not, and then, the propagation process can be viewed as a sequence of activation of nodes. A diffusion process occurring inside a network is characterized by two aspects: (i) its topology and (ii) its temporal dynamic.

==> intro_approach.tex <==
\textbf{Novelty and contributions.} Most of existing predictive models focus on the topology of the process and are based on uni-dimensional feature spaces. They intend to predict properties like the depth of the spreading cascade or the total size of the reached population and vastly ignore the temporal dimension. In this paper, we consider the issue of predicting the temporal dynamics of the diffusion process in online social networks. Our initial assumption is that the macroscopic dynamics of the spreading process are explained by the topology of the network and the interactions that occur through it, between pairs of users, on the basis of properties at the microscopic level. We thus base our approach on a multidimensional analysis of users behaviour, from which we derive a 3-dimensional feature list: (i) social, (ii) time and (iii) topic/semantic. To reproduce the diffusion phenomenon, we introduce a new graph-based model, the \textit{Time-Based Asynchronous Independent Cascades (T-BaSIC) model} whose parameters are functions of time and use machine learning techniques to estimate them.

==> twitter.tex <==
\textbf{Context of this study.} Mainly for availability reasons, we -- like the majority of studies that addresses the modeling of information diffusion in social networks and used non-synthetic data -- base the practical part of this paper on data from Twitter. This allows us to easily position and compare our approach with related work.
% Description of the structure of Twitter and how we mathematically represent it
Twitter\footnote{\url{http://www.twitter.com/}} is a micro-blogging service that allows its users to publish public directed or undirected short messages (140 characters at most) and to follow other users that interest them. Send a directed message is achieved by mentioning the targeted users directly in the content with the convention ``@username''. Both directed and undirected messages are automatically forwarded to the followers but directed messages aim more particularly at one or more specific users. Overall, Twitter forms an online social network where the information flows from place to place, in two different ways: (i) it flows in a passive manner via the following ties and also (ii) actively because of users that directly send information to others via the mentioning practice. Mathematically speaking we represent this network as a directed multigraph comprised of two sets of edges: (i) the set of following edges, which constitutes the \textit{passive} part of the network, commonly called ``follower graph''; (ii) the set of mentioning edges, that represents the \textit{active} part of the social network.

